Difference-in-Differences with Multiple Events

This paper studies staggered Difference-in-Differences (DiD) design when there is a second event confounding the target event. When the events are correlated, the treatment and the control group are unevenly exposed to the effects of the second event, causing an omitted event bias. To address this bias, I propose a two-stage DiD design. In the first stage, I estimate the combined effects of both treatments using a control group that is neither treated nor confounded. In the second stage, I isolate the effects of the target treatment by leveraging a parallel treatment effect assumption and a control group that is treated but not yet confounded. Finally, I apply this method to revisit the effect of minimum wage increases on teen employment using state-level hikes between 2010 and 2020. I find that the Medicaid expansion under the ACA is a significant confounder: controlling for this bias reduces the short-term estimate of the minimum wage effect by two-thirds.

==> paper/twoperiod.tex <==

\section{A Two-Period Setup.}
Let's first examine the omitted event bias in a simplified setting. Consider an otherwise canonical 2-by-2 with two events. There are $t = 1,2$ periods and $i = 1,..., N$ units. $D^1_i, D^2_i$ are binary variables that indicate if unit $i$ is treated by event 1 or event 2. For the potential outcomes \citep{Rubin1974-yt}, let $Y_{it}(g^1, g^2), g^1, g^2 \in\{0,1\}$ denote the potential outcome of unit $i$ in period $t$ if it is treated by event 1 or event 2. The relationship between observed and potential outcomes is determined by

\begin{align}
    \begin{split}
    Y_{it} = & \mathbbm{1}\{D^1_i = 0, D^2_i = 0\}Y_{it}(0,0) + \mathbbm{1}\{D^1_i = 1, D^2_i = 0\}Y_{it}(1,0) \\ & + \mathbbm{1}\{D^1_i = 0, D^2_i = 1\}Y_{it}(0,1) + \mathbbm{1}\{D^1_i = 1, D^2_i = 1\}Y_{it}(1,1).
    \end{split}
\end{align}

\noindent We define the treatment effect of event 1 as $Y_{i2}(1, 0) - Y_{i2}(0,0)$, the treatment effect of event 2 as $Y_{i2}(0, 1) - Y_{i2}(0,0)$, and of the combined treatment effect of event 1 and event 2 as $Y_{i2}(1, 1) - Y_{i2}(0,0)$. 

\bigskip

Throughout this paper, we assume that the researcher is interested in event 1 (the target event) but not event 2 (the confounding event) without loss of generality. We also treat the (pure) treatment effect of event 1 as the parameter of interest. This means that event 2 is not a causal mechanism of the interested effect of event 1, i.e., event 2 is not a bad control.

\bigskip

For the DiD design, let's assume that parallel trend holds for both events: $E[Y_{i2}(0,0)-Y_{i1}(0,0)|D^1_i, D^2_i] = E[Y_{i2}(0,0)-Y_{i1}(0,0)],$ and also no anticipation $E[Y_{i1}(g^1,g^2)|D^1_i, D^2_i] = E[Y_{i1}(0,0)|D^1_i, D^2_i], \forall \{g^1,g^2\} \in \{\{1,0\},\{0,1\},\{1,1\}\}$. To simplify the exposition, I also assume no treatment effect heterogeneity $ \mathbb{E}[Y_{i2}(g^1, g^2) - Y_{i2}(0,0)|D^1_i, D^2_i] = \mathbb{E}[Y_{i2}(g^1, g^2) - Y_{i2}(0,0)] \equiv ATT^{g^1g^2}\:, \forall \{g^1,g^2\} \in \{\{1,0\},\{0,1\},\{1,1\}\}.$ Under these conditions, the one-event DiD moment can be defined as:

\begin{equation*}
    ATT^{did} \equiv \mathbb{E}[Y_{i2} - Y_{i1} |D^1_i = 1] - \mathbb{E}[Y_{i2} - Y_{i1} |D^1_i = 0],
\end{equation*}

Under confounding events, it does not identify the average target treatment effect:

\begin{align}\label{eq:2b2}
\begin{split}
    ATT^{did}
    = & ATT^{10} + \underbrace{[ATT^{11} - ATT^{01} - ATT^{10}]P(D^2_i = 1|D^1_i = 1)}_{\text{interaction bias}} \\
    & + \underbrace{ATT^{01}[P(D^2_i=1|D^1_i = 1) - P(D^2_i=1|D^1_i = 0) ].}_{\text{omitted event bias}}
\end{split}
\end{align}

Expositions are collected in Appendix \ref{app:proof}
There are two sources of bias, the interaction bias and the omitted event bias. The interaction bias comes from the fact that the treatment effect of event 1 on neither treated $ATT^{10}$ may differ from the effect on those already treated by event 2 $ATT^{11} - ATT^{01}$. I can do little about it. 

\bigskip

The second is the omitted event bias. If two events are correlated ($P(D^2_i=1|D^1_i = 1) - P(D^2_i=1|D^1_i = 0)$), the treatment group will have different exposure to event 2 compared to the control group. As a result, the effect of the confounding event ($ATT^{01}$) breaks the parallel trend for event 1. The solution is simple: only use units treated by neither event as control:

\begin{equation*}
ATT^{did2} = \mathbb{E}[Y_{i2} - Y_{i1} |D^1_i = 1, D^2_i = 0] - \mathbb{E}[Y_{i2} - Y_{i1} |D^1_i = 0, D^2_i = 0].
\end{equation*}

This identifies the ATT10. Extends to multiple

==> paper/ztrash.tex <==
For using never-treated-by-other-event as control groups:


\begin{assumption}[Parallel Treatment Effects - Never-Treated]\label{ass:ptet-never}

    For $g^1 \in \mathbb{G}^1, g^2 \in \mathbb{G}^2, t\in \{1,...,T\}$, and $t$ such that $t\geq g^2$, 

    $$ATT^{01}(g^1, g^2, t) - ATT^{01}(g^1, g^2, g^1-1) = ATT^{01}(\infty, g^2, t) - ATT^{01}(\infty, g^2, g^1-1),$$ 
    
    and for $t$ such that $t\geq g^1$
    
    $$ATT^{10}(g^1, g^2, t) - ATT^{10}(g^1, g^2, g^2-1) = ATT^{10}(g^1, \infty, t) - ATT^{10}(g^1, \infty, g^2-1).$$
\end{assumption}


\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{source/observed.png} 
    \caption{Difference in Difference with Two Events}
    \label{fig:observed}
    \fnote{This figure illustrates a two-event setup with multiple periods and staggered cohort. The cohorts are indexed by $G^1, G^2$. The enlarged points are periods where a cohort is first treated by an event, and the number on top is the index ($d$) of the event. Each line represents the average outcomes of cohorts. The solid line is the realized outcome $Y$, and the dotted lines are $Y(G^1,0).$}
\end{figure}

==> slide/1-introduction.tex <==
\section{Introduction}

\AddButton

\begin{frame}{Confounding Treatment in 2x2 DiD}

    \begin{itemize}
        \item Card and Krueger (1993): NJ raised the minimum wage, PA didn't.
        \item Parallel trends without the hike $\implies ATT^{did} = ATT^1$. 
        \item What if NJ also expanded its social security ($ATT^{2}$)? 
    \end{itemize}
    
    \begin{align}\label{eq:2b2}
    \begin{split}
        ATT^{did} \equiv & \mathbb{E}[Y_{i2}-Y_{i1}|D^1_i=1] - \mathbb{E}[Y_{i2}-Y_{i1}|D^1_i=0] \\
        = & ATT^{1} + \underbrace{ATT^{2}[P(D^2_i=1|D^1_i = 1) - P(D^2_i=1|D^1_i = 0) ].}_{\text{omitted event bias}}. 
    \end{split}
    \end{align}
    \begin{itemize}
        \item 2x2: control for $D^2_i$.
        \item Staggered adoption? Treatment effect heterogeneity? 
    \end{itemize}
\end{frame}


\begin{frame}{Double DiD}

    Control confounding events w/ rich treatment effect heterogeneity
    \begin{itemize}
        \item Extend Callaway and Sant'Anna (2021) to Double-Group-Time ATT
        \item Identify the target treatment effect with Two-Stage DiD
        \begin{itemize}
            \item Omitted event bias in DiD: confounded controls and treated units
            \item First DiD: not-yet-treated-nor-confounded as control
            \item Second DiD: simultaneously-treated-but-not-yet-confounded as control under parallel treatment effect
        \end{itemize}
        \item Provide estimation, aggregation, inference: analogous to CS
        \item Obamacare created a spurious negative estimate of the effect of minimum wage on teen employment 
        \item Implementation: fastdid (R package)
    \end{itemize}

\end{frame}

\begin{frame}{Literature: Confounding Events in Staggered DiD}


    \begin{columns} 
    \begin{column}{.4\textwidth}
        \begin{figure}
     \includegraphics[width=1\textwidth]{source/lit.png} 
        \label{fig:lit}
    \end{figure}
    \end{column}
    \begin{column}{.6\textwidth}    

    \begin{itemize}
        \item TWFE: biased under heterogeneity (Goodman-Bacon, 2021) 
        \item Caetano and Callaway (2024): confounding treatment as time-varying covariate
        \item de Chaisemartin and D'Haultfoeuille (2023): common trend conditional on treatment status in $t-1$
        \item This paper: allow (own) cohort and time heterogeneity
    \end{itemize}

    \bigskip

    Contribution: most selective with cont. group $\rightarrow$ most flexible treatment effect het. 
          
        \end{column}
    \end{columns}
    
\end{frame}


    
  








==> slide/2-model.tex <==
\section{Setup}

\begin{frame}[label=exam]{Setup: Example}

\begin{figure}
 \includegraphics[width=0.6\textwidth]{source/setup.png} 
    \label{fig:observed}
\end{figure}

\end{frame}


\begin{frame}{Setup: CS with Two Treatments}

CS (2021) with a second treatment 
\begin{itemize}
    \item Panel with periods $t = 1,...,T$ and units $i = 1,...,N$ 
    \item Two treatments $d \in \{1,2\}$. $D^d_{it} \in \{0,1\}$.
    \item For multiple confounding treatments, set $D^2_{it} = \max(D^2_{it},..., D^R_{it})$.
    
\end{itemize}

\begin{assumption}[Irreversible Treatments]\label{ass:irrtreat}
    For $d = 1,2$, $D^d_1 = 0$ a.s. For $d = 1,2, t = 2,..,T$ $D^d_{t-1} = 1 \implies D^d_{t} = 1$.
\end{assumption}

\begin{itemize}
    \item event cohort is the period first treated: $G^d_i = \underset{D^d_{it} = 1}{\min} t$ (untreated $\rightarrow \infty$). 
    \item $D^1$: target event
    \item $D^2$: confounding event
\end{itemize}

\end{frame}

\begin{frame}{Setup: Potential Outcome}

Dynamic Potential Outcome (Murphy 2001):

\begin{equation}\label{eq:potout}
    Y_{it} = Y_{it}(0,0) + \sum^T_{g^1 = 2}\sum^T_{g^2 = 2}(Y_{it}(g^1, g^2)- Y_{it}(0, 0))G^1_{ig^1}G^2_{ig^2}.
\end{equation}

\begin{assumption}[Random Sampling]\label{ass:sample}
    $\{Y_{i1}, Y_{i2},...,Y_{iT}, X_i, D^1_{i1},D^1_{i2},...,D^1_{iT}, D^2_{i1},D^2_{i2},...,D^2_{iT}\}^N_{i=1}$ is i.i.d.
\end{assumption}

\begin{assumption}[Overlap]\label{ass:overlap}
    \textit{There are enough treated and not-yet treated units across all cohorts, time, and covariates values.}
\end{assumption}
     
\end{frame}


\begin{frame}{Setup: Anticipation}

Both treatments have no treatment effect before the event occurs.

\begin{assumption}[No Anticipation]\label{ass:anticipation}
    For $g^1\in \mathbb{G}^1, g^2\in \mathbb{G}^2, 1 \leq t < \max(g^1, g^2)$ 
    \begin{equation*}
        \mathbb{E}[Y_t(g^1, g^2)|X, G^1_{g^1} = 1, G^2_{g^2} = 1] = \begin{dcases*}
             \mathbb{E}[Y_t(0,0)|X, G^1_{g^1} = 1, G^2_{g^2} = 1], t < \min(g^1, g^2), \\
            \mathbb{E}[Y_t(g^1,0)|X, G^1_{g^1} = 1, G^2_{g^2} = 1], g^1\leq t <g^2, \\
            \mathbb{E}[Y_t(0,g^2)|X, G^1_{g^1} = 1, G^2_{g^2} = 1], g^2\leq t <g^1.
    \end{dcases*}  
    \end{equation*}

\end{assumption}
\end{frame}

\begin{frame}{Setup: Parallel Trend}

Untreated trend is parallel between treated and not-yet-treated-nor-confounded units. 

\begin{assumption}[Parallel Trends - Not-Yet-Treated]\label{ass:pt}
    For $g^1\in \mathbb{G}^1, g^2\in \mathbb{G}^2, t\in \{1,...,T\}$, and $(s,t)$ such that $t\geq \min(g^1, g^2)$, $t \leq s < \min(\bar{G^1}, \bar{G^2})$

    $$ \mathbb{E}[Y_t(0, 0) - Y_{t-1}(0, 0)|X, G^1_{g^1} = 1, G^2_{g^2} = 1] = $$
    $$ \mathbb{E}[Y_t(0, 0) - Y_{t-1}(0, 0)|X, D^1_s = 0, D^2_s = 0, G^1_{g^1} = 0, G^2_{g^2} = 0].$$
\end{assumption}
     
\end{frame}

\begin{frame}{Double-Group-Time Average Treatment Effect}

    Target parameter: Target treatment effect
    $$ATT^1(g^1, g^2, t) \equiv \mathbb{E}[Y_t(g^1, 0) - Y_t(0,0)|G_{g^1}^1 = 1, G_{g^2}^2 = 1].$$

    \bigskip

    Target of first DiD: Combined effect of treatment 1 and/or treatment 2 
    \begin{equation}\label{eq:attggt}
    ATT(g^1, g^2, t) \equiv \mathbb{E}[Y_t(g^1, g^2) - Y_t(0,0)|G_{g^1}^1 = 1, G_{g^2}^2 = 1].
    \end{equation}

    \bigskip

    Confounding treatment effect:
    $$ATT^2(g^1, g^2, t) \equiv \mathbb{E}[Y_t(0, g^2) - Y_t(0,0)|G_{g^1}^1 = 1, G_{g^2}^2 = 1].$$
     
\end{frame}







==> slide/3-identification.tex <==

\section{First DiD: Confounded Control}


\begin{frame}{Omitted Event Bias}

    \begin{columns} 
    \begin{column}{.5\textwidth}
        \begin{figure}
     \includegraphics[width=1\textwidth]{source/oeb.png} 
        \label{fig:observed}
    \end{figure}
    \end{column}
    \begin{column}{.5\textwidth}    

          $\textcolor{red}{ATT^{CS}(2,4)} = ATT^1(2,4,4) $  
          $- \textcolor{blue}{ATT^2(5,3,4)} + \textcolor{mygreen2}{ATT^2(2,4,4)}$ 

          \bigskip

          Bias from both \textcolor{blue}{confounded control} and \textcolor{mygreen2}{confounded treatment}.  
          
        \end{column}
    \end{columns}
\end{frame}


\begin{frame}{Theorem 1: Omitted Event Bias in DiD}

    \begin{theorem}\label{thm:gtbias}
    If for all $g^1, g^2, t$, $ATT^{1}(g^1, g^2, t) = ATT^{1}$, $ATT^{2}(g^1, g^2, t) = ATT^{2}$ and , $ATT(g^1, g^2, t) = ATT$ for all $g^1 \geq t, g^2 \geq t$, then, for $g^1 \in \mathbb{G}^1, t\in \{2,...,T\}$ such that $g^1\leq t < \bar{g}^1$,
    
    \begin{align*}
    ATT^{CS}(g^1, t) &  =  ATT^{1}(g^1, t) \\
    & + \underbrace{ATT^{2}\big\{\overbrace{P(D^2_t = 1, D^2_b = 0 | G^1_{g^1 }= 1)}^{\text{confounded treated}} -\overbrace{P(D^2_t = 1, D^2_b = 0 | D^1_t = 0 )}^{\text{confounded control}}\big\}}_{\text{omitted event bias}} \\
    & + \underbrace{\{ATT-ATT^{1}-ATT^{2}\} P(D^2_t = 1 | G^1_{g^1} = 1).}_{\text{interaction bias}}
\end{align*}
\end{theorem}
\end{frame}


\begin{frame}{First DiD}

    Use a control group not yet treated nor confounded ($D^1_t = 0, D^2_t = 0$). let $b = \min(g^1, g^2) -1$,
    
    \begin{align*}
    ATT_{unc}(g^1, g^2, t) \equiv & \mathbb{E}[Y_t - Y_{b}|G^1_{g^1} = 1, G^2_{g^2} = 1]  - \mathbb{E}[Y_t - Y_{b}|D^1_t = 0, D^2_t = 0] \\
    = & \mathbb{E}[Y_t(g^1, g^2)|G^1_{g^1} = 1, G^2_{g^2} = 1]  - \mathbb{E}[Y_b(0, 0)|G^1_{g^1} = 1, G^2_{g^2} = 1]  \\
    & - \mathbb{E}[Y_t(0, 0)- Y_{b}(0, 0)|D^1_t = 0, D^2_t = 0] \text{ (No Antic.)} \\
    = & \mathbb{E}[Y_t(g^1, g^2)- Y_t(0,0)|G^1_{g^1} = 1, G^2_{g^2} = 1] \text{ (PT)} \\
    = & ATT(g^1, g^2, t). 
\end{align*}
        
\end{frame}



\begin{frame}{The Combined Event}

\begin{columns} 
    \begin{column}{.5\textwidth}
        \begin{figure}
     \includegraphics[width=1\textwidth]{source/unconfound.png} 
        \label{fig:observed}
    \end{figure}
    \end{column}
    \begin{column}{.5\textwidth}    

         \begin{itemize}
            \item Combined event: $G = \min(G^1, G^2)$ 
            \item $G$ satisfies CS's assumptions in $i\in \mathbb{I}(g^1, g^2)$ 
            \item $\mathbb{I}(g^1, g^2)$: keep control group ($\min(G^1, G^2) > g$) and target treated ($G^1 = g^1, G^2 = g^2$). 
            \item Can use CS's result for conditional parameters (IPW, OR, DR)
        \end{itemize}
        
    \end{column}
\end{columns}
\end{frame}


\begin{frame}{Theorem 2: Ident. of Combined Treatment Effect}

\begin{theorem}\label{thm:ggtident}
For $g^1 \in \mathbb{G}^1, g^2 \in \mathbb{G}^2, t\in \{2,...,T\}$ such that $\min(g^1, g^2) \leq t < \min(\bar{g}^1, \bar{g}^2)$,

\begin{align}
    \begin{split}
        ATT(g^1, g^2, t) & = ATT_{unc}(g^1, g^2, t) = ATT_{ipw}(g^1, g^2, t) \\
        & = ATT_{or}(g^1, g^2, t) = ATT_{dr}(g^1, g^2, t).
    \end{split}
\end{align}
\end{theorem}

\end{frame}

\section{Second DiD: Confounded Treated}

\begin{frame}{Remaining Problem: Confounded Treated}

    \begin{columns} 
    \begin{column}{.5\textwidth}
        \begin{figure}
     \includegraphics[width=1\textwidth]{source/problem.png} 
        \label{fig:problem}
    \end{figure}
    \end{column}
    \begin{column}{.5\textwidth}    

          $G^1 < t < G^2: \textcolor{red}{ATT(2,\infty,2)} = ATT^{1}$  
          
          $G^1 < G^2 < t: \textcolor{blue}{ATT(2,4,4)} = ATT$ 
          
          $G^2 < G^1 < t: \textcolor{myyellow}{ATT(5,2,5)} = ATT$ 
          
          $G^2 < t < G^1: \textcolor{mygreen2}{ATT(5,2,3)} = ATT^{2}$ 

          \bigskip

          Goal: impute the missing treatment effects with a second DiD
          
    \end{column}
\end{columns}

\end{frame}

\begin{frame}{Parallel Treatment Effect}

Within simultaneously-treated units ($g^1$), $ATT^1$ is parallel between confounded and not-yet-confounded units ($g^2$). 

\begin{assumption}[Parallel Treatment Effects]\label{ass:ptet}

    For $g^1 \in \mathbb{G}^1, g^2 \in \mathbb{G}^2, t\in \{1,...,T\}$, $t\geq g^1$, $t \leq s^2$,
    $$ATT^{1}(g^1, g^2, t) - ATT^{1}(g^1, g^2, g^2-1) = ATT^{1}(g^1, s^2, t) - ATT^{1}(g^1, s^2, g^2-1),$$

    and vice versa for $ATT^2$ within $g^2$ across $g^1$. 
    
\end{assumption}

\begin{assumption}[No Interaction]\label{ass:addeff}
    $$ATT(g^1, g^2, t) = ATT^{1}(g^1, g^2, t) + ATT^{2}(g^1, g^2, t).$$
\end{assumption}

\end{frame}

\begin{frame}{Imputation}

\begin{columns} 
    \begin{column}{.6\textwidth}
        \begin{figure}
        \includegraphics[width=1\textwidth]{source/impute.png} 
            \label{fig:impute}
        \end{figure}
    \end{column}
    \begin{column}{.4\textwidth}

        Treated-then-confounded: 
        \begin{itemize}
            \item control: not-yet-confounded
            \item impute $ATT^1$
        \end{itemize}
        \begin{align*}
            & ATT^{1}(2,4,4) =  \textcolor{blue}{ATT(2,\infty,4)} \\
            & + \textcolor{red}{ATT(2,4,3)} - \textcolor{mygreen2}{ATT(2,\infty,3)}
        \end{align*}
    \end{column}
\end{columns}
\end{frame}

\begin{frame}{Imputation}

\begin{equation}\label{eq:imp}
    ATT^{imp}_{id}(\tilde{g}^1, \tilde{g}^2, \tilde{t}) = \sum_{g^1\in \mathbb{G}^1}\sum_{g^2\in \mathbb{G}^2}\sum_{t=2}^Tw^{imp}_{\tilde{g}^1, \tilde{g}^2, \tilde{t}}(g^1, g^2, t)ATT_{id}(g^1, g^2, t),
\end{equation}

\begin{equation*}
    w^{imp}_{\tilde{g}^1, \tilde{g}^2, \tilde{t}}(g^1, g^2, t) \equiv \begin{dcases*}
    1, & if $t = \tilde{t}, g^1 = \tilde{g}^1, g^2 = \tilde{g}^2$, \\
    P(G^2_{g^2}=1 | G^1_{g^1} = 1, D^2_t = 0), & if $g^1 = \tilde{g}^1, g^2 > \tilde{t}, t = \tilde{t}$,\\
    -P(G^2_{g^2}=1 | G^1_{g^1} = 1, D^2_t = 0), & if $g^1 = \tilde{g}^1, g^2 > \tilde{t}, t = \tilde{g}^2-1$,\\
    0 & else.
    \end{dcases*} 
\end{equation*}

\end{frame}



\begin{frame}{DiD}

\begin{columns} 
    \begin{column}{.6\textwidth}
        \begin{figure}
        \includegraphics[width=1\textwidth]{source/ddid.png} 
           \label{fig:ddid}
        \end{figure}
    \end{column}
    \begin{column}{.4\textwidth} 
    
        Confounded-then-treated: 
        \begin{itemize}
            \item control: not-yet-treated 
            \item impute $ATT^2$
            \item $ATT^1 = ATT - ATT^2$
        \end{itemize}
        \begin{align*}
            & ATT^{1}(5,3,5) = \\
            & \textcolor{red}{ATT(5,3,5)} - \textcolor{blue}{ATT(5,3,4)} \\
            & - (\textcolor{mygreen2}{ATT(\infty,3,5)} - \textcolor{myyellow}{ATT(\infty,3,4)})
        \end{align*}
    \end{column}
\end{columns}
\end{frame}

\begin{frame}{DiD}

\begin{equation}\label{eq:did}
    ATT^{did}_{id}(\tilde{g}^1, \tilde{g}^2, \tilde{t}) = \sum_{g^1\in \mathbb{G}^1}\sum_{g^2\in \mathbb{G}^2}\sum_{t=2}^Tw^{did}_{\tilde{g}^1, \tilde{g}^2, \tilde{t}}(g^1, g^2, t)ATT_{id}(g^1, g^2, t),
\end{equation}

\begin{equation*}
    w^{did}_{\tilde{g}^1, \tilde{g}^2, \tilde{t}}(g^1, g^2, t) \equiv \begin{dcases*}
    1, & if $t = \tilde{t}, g^1 = \tilde{g}^1, g^2 = \tilde{g}^2$, \\
    -1, & if $t = \tilde{g}^1-1, g^1 = \tilde{g}^1, g^2 = \tilde{g}^2$, \\
    -P(G^1_{g^1}=1 | G^2_{g^2} = 1, D^1_t = 0), & if $g^1 > t, g^2 = \tilde{g}^2, t = \tilde{t}$,\\
    P(G^1_{g^1}=1 | G^2_{g^2} = 1, D^1_t = 0), & if $g^1 > t, g^2 = \tilde{g}^2, t = \tilde{g}^1-1$,\\
    0 & else.
    \end{dcases*} 
\end{equation*}
\end{frame}

\begin{frame}{Double DiD}

Given an identifying moment $ATT_{id}$ from Theorem 2, with DiD ($ATT^{did}$), Imputation ($ATT^{imp}$), and direct observation, we can identify $ATT^1$ in periods with discrepancies in treatment timing and suitable control groups. 

\begin{equation}\label{eq:ddid}
    ATT^{dd}_{id}(g^1, g^2, t) \equiv \begin{dcases*}
    ATT_{id}(g^1, g^2, t), & if $ t < g^2 $, \\
    ATT^{imp}_{id}(g^1, g^2, t), & if $ t \geq g^2$ and $g^1 < g^2$,\\
    ATT^{did}_{id}(g^1, g^2, t), & else.
    \end{dcases*}  
\end{equation}


\end{frame}


\begin{frame}{Theorem 3: Ident. of Target Treatment Effect}

\begin{theorem}\label{thm:doubledid}
 Under assumption \ref{ass:ptet} and \ref{ass:addeff}, for an identifying moments $ATT_{id}$ such that $ATT_{id} = ATT$, for all $g^1, g^2, t$ such that (1) $g^1 < g^2$, $g^1 \leq t < \bar t^1$, or (2) $g^1 > g^2$, $g^1 \leq t < \bar t^2$,

\begin{align*}
ATT^{1}(g^1, g^2, t) = ATT^{dd}_{id}(g^1, g^2, t),
\end{align*}

 
\end{theorem}

\end{frame}


\begin{frame}{Aggregation, Estimation and Inference}

Aggregation (group-time, dynamics, simple, ...):
\begin{equation}\label{eq:agg}
    \theta = \sum_{g^1\in \mathbb{G}^1}\sum_{g^2\in \mathbb{G}^2}\sum_{t=2}^Tw(g^1, g^2, t)ATT^1(g^1, g^2, t).
\end{equation}

\bigskip

Estimation and Inference
\begin{itemize}
    \item First DiD (DGTATT)
    \begin{itemize}
        \item estimation: CS' GTATT on the subsample $\mathbb{I}(g^1, g^2)$
        \item inference follows
    \end{itemize}
    \item Second DiD (Imputation, DiD)
     \begin{itemize}
        \item identification: a summary parameter of DGTATT
        \item estimation and inference follows
    \end{itemize}
\end{itemize}



\end{frame}



==> slide/5-empirical.tex <==
\section{Empirical Application}

\begin{frame}{Minimum Wage and ACA Medicaid Expansion}

Minimum Wage on Employment
\begin{itemize}
    \item 2-by-2: Card and Krueger (1994)
    \item State-Year TWFE: Neumark (2006)
    \item New DiD: Callaway and Sant'Anna (2021) $\rightarrow$ Teen Employment
\end{itemize}

\bigskip

Confounding Policy with Minimum Wage
\begin{itemize}
    \item States that increase the minimum wage may also adopt other policies.
    \item Example: Medicaid Expansion under ACA (Obamacare)
    \item $\rightarrow$ Is minimum wage on teen employment confounded by ACA?
\end{itemize}

\end{frame}

\begin{frame}{Confoundedness between Minimum Wage and ACA}


\begin{columns} 
    \begin{column}{.5\textwidth}
        \begin{figure}
            \centering
            \includegraphics[width=1\textwidth]{source/diag_never.png} 
            \label{fig:diag}
        \end{figure}
    \end{column}
    \begin{column}{.5\textwidth} 
            No pre-tend in treatment
            
            $\rightarrow$ no pre-trend in the outcome!
    \end{column}
\end{columns}


\end{frame}

\begin{frame}{Omitted Event Bias}

\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{source/es_main.png} 
    \label{fig:est}
\end{figure}


\end{frame}

\begin{frame}{Discussion}


Interpretation
\begin{itemize}
    \item ACA lowered teen employment? Minimum wage have no effect?
    \item No. State-year is underpowered, Confounding policy is everywhere. 
    \item Takeaway: omitted event bias matters. 
\end{itemize}

\bigskip

\centering{Thank you!}

\end{frame}
